Requirements Quality vs Process and Stakeholders' Well-being: A Case of a Nordic Bank

Requirements are key artefacts to describe the intended purpose of a software system. The quality of requirements is crucial for deciding what to do next, impacting the development process's effectiveness and efficiency. However, we know very little about the connection between practitioners' perceptions regarding requirements quality and its impact on the process or the feelings of the professionals involved in the development process. Objectives: This study investigates: i) How software development practitioners define requirements quality, ii) how the perceived quality of requirements impact process and stakeholders' well-being, and iii) what are the causes and potential solutions for poor-quality requirements. Method: This study was performed as a descriptive interview study at a sub-organization of a Nordic bank that develops its own web and mobile apps. The data collection comprises interviews with 20 practitioners, including requirements engineers, developers, testers, and newly employed developers, with five interviewees from each group. Results: The results show that different roles have different views on what makes a requirement good quality. Participants highlighted that, in general, they experience negative emotions, more work, and overhead communication when they work with requirements they perceive to be of poor quality. The practitioners also describe positive effects on their performance and positive feelings when they work with requirements that they perceive to be good.

==> tables/qualities.tex <==
\begin{table}[]
\begin{tabular}{llllll}
Code                      & Requirements Engineers & Testers & Developers & Recently-Recruited Developers & Total \\
Clear                     & 5                      & 5       & 5          & 5                             & 20    \\
Complete                  & 2                      & 5       & 5          & 5                             & 17    \\
Pupose                    & 5                      & 2       & 3          & 2                             & 12    \\
Relevant for stakeholders & 2                      & 2       & 4          & 0                             & 8     \\
Short description         & 3                      & 2       & 1          & 2                             & 8     \\
Well structured           & 2                      & 3       & 0          & 2                             & 7     \\
Concrete                  & 3                      & 2       & 2          & 0                             & 7     \\
Correct                   & 0                      & 1       & 1          & 2                             & 4     \\
Easy to adjust            & 1                      & 1       & 1          & 1                             & 4     \\
Testable                  & 0                      & 2       & 1          & 1                             & 4     \\
Terminology               & 2                      & 1       & 0          & 0                             & 3     \\
Feasible                  & 1                      & 0       & 0          & 2                             & 3     \\
Logical                   & 1                      & 0       & 0          & 1                             & 2     \\
Not-an-epic               & 0                      & 0       & 2          & 0                             & 2     \\
Not-too-detailed          & 0                      & 0       & 1          & 0                             & 1     \\
Traceable                 & 1                      & 0       & 0          & 0                             & 1    
\end{tabular}
\end{table}
